Co-scheduling Ensembles of In Situ Workflows

Molecular dynamics (MD) simulations are widely used to study large-scale molecular systems. HPC systems are ideal platforms to run these studies, however, reaching the necessary simulation timescale to detect rare processes is challenging, even with modern supercomputers. To overcome the timescale limitation, the simulation of a long MD trajectory is replaced by multiple short-range simulations that are executed simultaneously in an ensemble of simulations. Analyses are usually co-scheduled with these simulations to efficiently process large volumes of data generated by the simulations at runtime, thanks to in situ techniques. Executing a workflow ensemble of simulations and their in situ analyses requires efficient co-scheduling strategies and sophisticated management of computational resources so that they are not slowing down each other. In this paper, we propose an efficient method to co-schedule simulations and in situ analyses such that the makespan of the workflow ensemble is minimized. We present a novel approach to allocate resources for a workflow ensemble under resource constraints by using a theoretical framework modeling the workflow ensemble's execution. We evaluate the proposed approach using an accurate simulator based on the WRENCH simulation framework on various workflow ensemble configurations. Results demonstrate the significance of co-scheduling simulations and in situ analyses that couple data together to benefit from data locality, in which inefficient scheduling decisions can lead up to a factor 30 slowdown in makespan.

==> src/sec-applications.tex <==
\section{Applications}
\label{sec:applications}

\subsection{Molecular Dynamics (MD) Simulation}
\label{subsec:md_simulation}
Molecular dynamics (MD) simulation discovers the behavior of a molecular system through computing the atomic positions that evolves over time to traverse the configuration space. 
Trajectory is a sequence of frames, which are snapshots of atomic coordinates, generated in a specific duration.  
Hence, in the remaining text of this paper, trajectory is the term to indicate the execution of a simulation of a molecular system in a certain amount of time in terms of number of simulation steps, which explicitly determines the trajectory length.

The number of computations of a given trajectory does not depend on the state, which region in the simulation space, being explored. 
More specifically, an MD step takes roughly the same amount of FLOPS (floating point computing per second) and CPU time no matter what the state of the simulated molecular system is.
Hence, time to simulate a trajectory is proportional to the timescale (i.e. number of simulation steps) and inversely proportional to the amount of assigned resources.

\subsection{In Situ Analyses}
\label{subsec:in_situ_analyses}
The insight of a molecular system is obtained by analyzing long enough trajectory generated by the simulation. 
The longer timescales are obtainable by the simulation, the larger the trajectories data needs to be stored for processing.
The data footprint is therefore considerable, which forms the challenges due to the slow growth of disk write rate compared to computational growth that marks the stagnation of file system throughput~\cite{ian2017}. 
In situ methods allow processing data during the runtime of the simulation to considerably reduce the final amount of data generated by the simulation by choosing on-the-fly which data are more essential to keep.
From scientific contributions, the essence of performing analyses online helps to study insights into phenomena of the molecular system in a timely fashion or lessen the burden on post-hoc processing.

% Metadynamics, collective variables
On the other hand, since trajectories are kept under high-dimensional objects while some motions are redundant to maintain in frames, there are attempts to only preserve a subset of selective information. 
Collective variables (CV) is defined as a function of a frame to reconstruct free energy surface into a smaller CV space for further analysis. 
The analysis of completed trajectories is more lightweight and efficient as collective variables are computed in situ.
Calculating CVs is well-suited to perform as in situ tasks along with the simulation.
\tu{Add references}
Combining with adaptive sampling introduced in the next section, sampling is enhanced to accelerate the convergence to region of interest.

% \subsection{Adaptive Sampling}
% Adaptive sampling is an iterative process in which each iteration restarts a set of simulations based on the analysis of trajectories explored in the previous iteration to efficiently reach the region of interest.
% Adaptive sampling offers a powerful approach to explore unknown high-dimensional parameter space.
% Adaptive sampling can be combined with enhance sampling methods to generate new simulations for much more efficient sampling.
% The advantages of adaptive sampling reply on two-fold: (1) speeding-up simulation time to specific rare events; (2)
% broadening exploration of the conformational space.
% Using adaptive sampling, it is not possible to a priori determine the number of iterations or input values for all iterations.

% \subsubsection{Execution scenarios}

% \begin{figure}[!ht]
% 	\centering
%     \begin{subfigure}[b]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{synchronous}
%         \caption{Synchronous manner}
%         \label{fig:synchronous}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{asynchronous}
%         \caption{Asynchronous manner}
%         \label{fig:asynchronous}
%     \end{subfigure}
%     \caption{Adaptive sampling manner}
%     \label{fig:adaptive_sampling}
% \end{figure}

==> src/sec-scheduling.tex <==
\section{Co-scheduling}
\label{sec:scheduling}

\subsection{Co-scheduling Strategies}
\label{subsec:co-scheduling}
In this section, we propose a greedy algorithm (see~\cref{alg:cosched}) to find a good co-scheduling partition $\{P^C,P^{NC}\}$. 
By initializing with the ideal partition where all analyses are co-scheduled with their coupled simulations, i.e. $P^C = A$ and $P^{NC} = \O$, the procedure greedily moves the analyses from $P^C$ to $P^NC$ and check the feasibility of such the co-scheduling partition iteratively until finding a sustainable partition.
~\cref{alg:feasi} describes the process of verifying the amount of resources to accommodate the co-scheduling partition
~\cref{tr:gm} confirms the termination condition of the algorithm as the process is not needed to proceed after a sustainable partition is found.

% \begin{theorem}
% \label{tr:gm}
% Not co-scheduling an analysis with its coupled simulation yields a greater minimized makespan. 
% \end{theorem}
% \begin{proof}
% We compare the minimal makespan of two following co-scheduling mappings: (1) the original co-scheduling mapping $m$ which corresponds to a co-scheduling partition $\{P^{C},P^{NC}\}$ and (2) the co-scheduling mapping $m'$ forming by moving an analysis $A_k$ from $P^{C}$ to $P^{NC}$, or corresponding to a new co-scheduling partition $P'^{C},P'^{NC}$ where $P'^{C} = P^{C} \setminus A_k$ and $P'^{NC} = P^{NC} \cup A_k$. 

% Since $A_k \in P^C$ in the co-scheduling $m$, i.e. the analysis is co-scheduled with its coupled simulation, the makespan of the co-scheduling mapping $m$, is minimized, denoted by $t$ when:
% \begin{align}
%     \label{eq:tak}
%     t &= T(A_k) = \frac{t_{A_k}(1)}{n_{A_k}c_{A_k}} 
% \end{align}
% While $A_k \in P'^{NC}$ or the analysis is not co-scheduled with its coupled simulation $S^k = p^{-1}(A_k)$ in the co-scheduling $m'$, the makespan is minimized at $t'$ when: 
% \begin{align}
%     \label{eq:t'ak}
%     t' &= T'(A_k) = \frac{t_{A_k}(1)}{n'_{A_k}c'_{A_k}} + \frac{V_{S^k}}{Bn'_{A_k}}
% \end{align}
% Let assume $t \geq t'$, then $T(A_k) \geq T'(A_k)$. From~\cref{eq:tak,eq:t'ak}, we have:
% \begin{align}
%     \frac{t_{A_k}(1)}{n_{A_k}c_{A_k}} &\geq \frac{t_{A_k}(1)}{n'_{A_k}c'_{A_k}} + \frac{V_{S^k}}{Bn'_{A_k}} > \frac{t_{A_k}(1)}{n'_{A_k}c'_{A_k}} \nonumber \\
%     &n_{A_k}c_{A_k} < n'_{A_k}c'_{A_k} \label{eq:r}
% \end{align}
% Let $r(X) = n_X c_X$ denote the amount of resources in terms of cores assigned to $X$.
% ~\cref{eq:r} indicates more resources assigned to $A_k$ in $m'$ than $m$. 
% However, as the total number of cores is limited to $NC$, in the co-scheduling $m'$, there must exist an application $I$ which is either a simulation in $S$ or an analysis in $A \setminus A_k$ such that it is assigned fewer resource than it is in the co-scheduling $m$. 
% Hence, $T'(X) > T(X)$ or $t' > t$, which is contradicted to our assumption. 
% \end{proof}


\begin{algorithm}
    \caption{\cosched Algorithm}\label{alg:cosched}
    \DontPrintSemicolon
    \Input{$S,A,N,C$}
    \Output{$P^{C}, P^{NC}, n^*, c^*$}
    $P^{C} \gets A$\;
    $P^{NC} \gets \O$\;
    \While{$P^C \neq \O$}{
        $n,c \gets \Fcoalloc(S,P^{C},P^{NC})$\;
        $R \gets \Ffeasible(n,c)$\;
        \eIf{$R' \neq \O$}{
            $P^C \gets P^C \setminus R$\;
            $P^{NC} \gets P^{NC} \cup R$\;
        }{
            $t \gets T(S,P^C,P^{NC})$\;
            \textbf{break}\;
        }
    }
    \Return{$(t,n,c,P^C,P^{NC})$}
\end{algorithm}

\begin{algorithm}
    \caption{Feasibility Checking}\label{alg:feasi}
    \DontPrintSemicolon
    \Fn{\Ffeasible($S,P^C,P^{NC}$)}{
        \Input{$S,P^C,P^{NC}$}
        \Output{}
        $R \gets \O$\;        
        \For{$S_i \in S \cup \nosim$}{ 
            $sum \gets 0$\;
            \lIf{$S_i \neq \nosim$}{
                $sum \gets m_{S_i}$\;
            }
            \For{$A_j \in p(S_i) \cap P^C$}{
                $sum \gets sum + m_{A_j}$\;
            }
            \If{$sum > M$}{
                $R \gets R \cup \Forder(p(S_i) \cap P^C)$\;
            }
        }
        \Return{$R$}\;
    }
\end{algorithm}


\note{Explain a little bit deeper the algorithms (slightly more details and don't hesitate to cite lines (you can with labels))}

% \subsection{Optimal Solution}
% \begin{algorithm}
%     \caption{Brute-force Algorithm}\label{alg:bfa}
%     \DontPrintSemicolon
%     \Input{$S,A,N,C$}
%     \Output{$P^{*C}, P^{*NC}, n^*, c^*$}
%     $t^* \gets +\infty$\;
%     \For{$P^{NC} \in  AC$}{
%         $P^{C} \gets A \setminus P^{NC}$\;
%         $n,c \gets \Fcoalloc(S,P^{C},P^{NC})$\;
%         $R \gets \Ffeasible(n,c)$\;
%         \If{$R' = \O$}{
%             $t \gets T(S,P^C,P^{NC})$\;
%             \If{$t < t^*$}{
%                 $t^* \gets t$\;
%                 $P^{*C} \gets P^{C}$\;
%                 $P^{*NC} \gets P^{NC}$\;
%                 $n^* \gets n$\;
%                 $c^* \gets c$\;
%             }
%         }
%     }
%     \Return{$(t^*,n^*,c^*,P^{*C},P^{*NC})$}\;
% \end{algorithm}

\subsection{Complexity Analysis}
